Cloud-by-cloud Multiphase Investigation of the Circumgalactic Medium of Low-redshift Galaxies

The pervasive presence of warm gas in galaxy halos suggests that the circumgalactic medium (CGM) is multiphase in its ionization structure and complex in its kinematics. Some recent state-of-the-art cosmological galaxy simulations predict an azimuthal dependence of CGM metallicities. We investigate the presence of such a trend by analyzing the distribution of gas properties in the CGM around 47 $z <$ 0.7 galaxies from the Multiphase Galaxy Halos Survey determined using a cloud-by-cloud, multiphase, ionization modelling approach. We identify three distinct populations of absorbers: cool clouds ($T \sim$ 10$^{4.1}$ K) in photoionization equilibrium, warm-hot collisionally ionized clouds ($T \sim$ 10$^{4.5-5}$ K) affected by time-dependent photoionization, and hotter clouds ($T \sim$ 10$^{5.4-6}$ K) with broad OVI and Lya absorption consistent with collisional ionization. We find that fragmentation can play a role in the origin of cool clouds, that warm-hot clouds are out of equilibrium due to rapid cooling, and that hotter clouds are representative of virialized halo gas in all but the lowest mass galaxies. The metallicities of clouds do not depend on the azimuthal angle or other galaxy properties for any of these populations. At face value, this disagrees with the simplistic model of the CGM with bipolar outflows and cold-mode planar accretion. However, the number of clouds per sightline is significantly larger close to the minor and major axes. This implies that the processes of outflows and accretion are contributing to these CGM cloud populations, and our sightlines are probing gas of mixed origins at all azimuthal angles in these low redshift galaxies.

==> Tables/summarystatistics_galaxy.tex <==
\begin{table}
\begin{center}
\caption{\bf Summary statistics of the galaxy properties associated with different cloud types}
\label{tab:summarystat_galaxy}

\begin{tabular}{ |c|c|c|c| } \hline

 Property & Cloud type & Median $\pm$ 1$\sigma$ & IQR\\\hline
 {\mhalo} & PIE & $11.93 \pm 0.03$ & [$11.66, 12.51$]\\
  & TDP--Low  & $11.87 \pm 0.05$ & [$11.79, 11.99$]\\
  & TDP--High  & $11.88 \pm 0.06$ & [$11.68, 12.09$]\\\hline
 {\coldenu} & PIE & $15.6 \pm 0.1$ & [$14.0, 16.6$]\\
  & TDP--Low  & $14.4 \pm 0.2$ & [$13.8, 15.5$]\\
  & TDP--High  & $12.9 \pm 0.1$ & [$12.5, 13.3$]\\\hline
 {\totalcoldenu} & PIE & $17.6 \pm 0.1$ & [$16.4, 18.5$]\\
  & TDP--Low  & $18.5 \pm 0.1$ & [$18.2, 18.8$]\\
  & TDP--High  & $19.2 \pm 0.1$ & [$18.6, 19.8$]\\\hline  
  {\tempu} & PIE & $4.11 \pm 0.03$ & [$4.0, 4.3$]\\
  & TDP--Low  & $4.62 \pm 0.06$ & [$4.4, 5.0$]\\
  & TDP--High  & $5.71 \pm 0.04$ & [$5.6, 5.9$]\\\hline  
  {\btherm} [{\kms}]  & PIE & $14.7 \pm 0.4$ & [$13.0, 18.2$]\\
  & TDP--Low  & $26.3 \pm 2.1$ & [$21.2, 42.5$]\\
  & TDP--High  & $89.8 \pm 5.6$ & [$76.5, 119.7$]\\\hline  
    {\bturb} [{\kms}]  & PIE & $11.4 \pm 1.5$ & [$5.7, 23.8$]\\
  & TDP--Low  & $25.8 \pm 2.3$ & [$16.0, 31.7$]\\
  & TDP--High  & $24.8 \pm 3.7$ & [$13.1, 45.4$]\\\hline
    {\bnet} [{\kms}]  & PIE & $21.3 \pm 1.2$ & [$15.5, 33.5$]\\
  & TDP--Low  & $38.0 \pm 2.1$ & [$33.9, 48.7$]\\
  & TDP--High  & $95.0 \pm 5.7$ & [$80.7, 123.9$]\\\hline
      {\hdenu}   & PIE & $-2.5 \pm 0.1$ & [$-2.8, -1.6$]\\
  & TDP--Low  & $-3.5 \pm 0.4$ & [$-4.4, -2.2$]\\
  & TDP--High  & {\nodata} & {\nodata}\\\hline
       {\thicknessu}   & PIE & $-1.4 \pm 0.2$ & [$-2.9, -0.4$]\\
  & TDP--Low  & $0.7 \pm 0.4$ & [$-1.2, 1.5$]\\
  & TDP--High  & {\nodata} & {\nodata}\\\hline
\end{tabular} \\
\end{center}
\end{table}
